Property Checking By Logic Relaxation

We introduce a new framework for Property Checking (PC) of sequential circuits. It is based on a method called Lo-gic Relaxation (LoR). Given a safety property, the LoR method relaxes the transition system at hand, which leads to expanding the set of reachable states. For j-th time frame, the LoR method computes a superset A_j of the set of bad states reachable in j transitions only by the relaxed system. Set A_j is constructed by a technique called partial quantifier elimination. If A_j does not contain a bad state and this state is reachable in j transitions in the relaxed system, it is also reachable in the original system. Hence the property in question does not hold. The appeal of PC by LoR is as follows. An inductive invariant (or a counterexample) generated by LoR is a result of computing the states reachable only in the relaxed system. So, the complexity of PC can be drastically reduced by finding a "faulty" relaxation that is close to the original system. This is analogous to equivalence checking whose complexity strongly depends on how similar the designs to be compared are.

==> junk.tex <==
\vspace{20pt}
just something to fill out the page
\clearpage
just something to fill out the page
\clearpage


==> o2_t2wo_imp_mods.tex <==
\section{Two Important Modifications Of \alg}
\label{sec:two_mods}
In this section, we consider two modifications of the \Alg algorithm
described in Section~\ref{sec:alg_descr}. The first modification is to
incorporate a ``manual'' relaxation that exploits the semantics of the
system.  The second modification is to combine a manual relaxation
with the machinery of inductive clauses of IC3. Sequential equivalence
checking is a promising application of this modification.

\subsection{Relaxation by an educated guess}
\label{subsec:str_awe_rlx}
In this subsection, we describe a modification of \Alg that starts
building a boundary formula $H_j$ by a relaxation that is just a guess
tailored to a particular class of systems/properties.  An example of
such a relaxation is given in Section~\ref{sec:exmp}.  The pseudo-code
of modified \Alg is given in Figure~\ref{fig:str_ind_rlx}. The only
difference between the original version shown in Fig.~\ref{fig:pc_lor}
and the modified one is in line 5 where function $\mi{EducatGuessRlx}$
is called instead of setting $H_j$ to 1. This function does the
following.  First it represents the original transition relation
$T_{j-1,j}$ as $\trx{j-1,j} \wedge R_{j-1,j}$. Here \trx{j-1,j} is the
relaxed transition relation replacing $T_{j-1,j}$.  Then
$\mi{EducatGuessRlx}$ calls a PQE solver to build a formula $H_j$ such
that $\prob{\Abs{W}{j-1}}{I_0 \wedge \Abs{H}{j-1} \wedge \Ttrx{j-1,j}
  \wedge R_{j-1,j}} \equiv H_j \wedge \prob{\Abs{W}{j-1}}{I_0 \wedge
  \Abs{H}{j-1} \wedge \Ttrx{j-1,j}}$. Here \Ttrx{j-1,j} is equal to
$\Ttrx{j-2,j-1} \wedge \trx{j-1}$.

\input{s3tr_aware_rlx.fig}
\subsection{Combining LoR with machinery of inductive clauses}
\label{subsec:lor_ic3}
In this subsection, we describe an algorithm called \Mix that combines
LoR and the machinery of inductive clauses used by IC3~\cite{ic3}. (IC
stands for Inductive Clauses.) The essence of IC3 is to build a
sequence of formulas $F_0,\dots,F_j$ where $F_0 = I_0$ and $F_k$,~$0 <
k \leq j$ over-approximates the set of states reachable in $k$
transitions. Eventually one of the over-approximating formulas turns
into an inductive invariant.  Formula $F_k$ is built by tightening
property $P$ with inductive clauses.  A clause $C$ is called
\tb{inductive} with respect to formula $F_k(S_k)$ if $F_k \wedge
C(S_k) \wedge T_{k,k+1} \rightarrow C(S_{k+1})$ holds.  If an
inductive invariant is ``far away'' from $P$ such a strategy may
perform poorly. In Section~\ref{sec:exmp}, we argued that sequential
equivalence checking is a PC example where IC3 may run into this
problem.

\input{m1ixed_alg.fig}

Algorithm \Mix is meant to cure the problem of IC3 above.  The main
difference of \Mix from IC3 is that an inductive invariant is built by
tightening a formula that is already significantly constrained with
respect to $P$ rather than $P$ itself.  The pseudo-code of \Mix is
given in Figure~\ref{fig:pc_lor_ic}.  It builds formulas
$H_0,\dots,H_j$ satisfying the CO conditions listed in
Subsection~\ref{subsec:co_conds} but does it differently from both
\Alg and IC3.  The lines marked with an asterisk differentiate \Mix
and IC3. Instead of initializing formula $H_j$ to $P$ as in IC3, \Mix
does the following (lines 5-6). First, \Mix calls function
$\mi{EducatGuessRlx}$ described in
Subsection~\ref{subsec:str_awe_rlx}. This function relaxes $T_{j-1,j}$
and builds a formula $H_j$ that makes up for the difference between
original and relaxed transition relations.  Then \Mix conjoins $H_j$
with $P$ (line 6). So $H_j$ is initialized to formula $P$ constrained
by the clauses returned by $\mi{EducatGuessRlx}$ rather than $P$ alone
as in IC3.

At this point, $H_j$ satisfies the first and second CO conditions. The
first CO condition i.e. \impl{I}{H_j} is satisfied due to \impl{I}{P}
and the stuttering feature (see
Subsection~\ref{subsec:one_two_conds}). The second CO condition
i.e. \impl{H_j}{P} is trivially satisfied due to the fact that $H_j$
contains the clauses of $P$ (added in line 6).

To satisfy the third CO condition, \Mix calls function
\SUb{ThirdCOcond}{IC}.  In contrast to $\mi{ThirdCOcond}$ of \alg,
\SUb{ThirdCOcond}{IC} does the job by inductive clauses. Suppose that
one needs to eliminate an $H_{j-1}$-state \pnt{s_{j-1}} from which a
state \pnt{s_j} falsifying $H_{j}$ is reachable in one transition.
Then $\SUb{ThirdCOcond}{IC}$ generates a clause inductive with respect
to $H_{j-1}$ that is falsified by \pnt{s_{j-1}} and adds it to
$H_{j-1}$.  Note that since $H_j$ is initialized in IC3 to $P$,
\pnt{s_j} is always a bad state. In \mix, \pnt{s_j} can be good as
well since $H_j$ is obtained by constraining $P$ with clauses returned
by $\mi{EducatGuessRlx}$. If \pnt{s_j} is a bad state and
\SUb{ThirdCOcond}{IC} fails to exclude \pnt{s_{j-1}}, it returns a
counterexample. In line 9, \Mix calls function \SUb{FinTouch}{IC} that
serves the same purpose as $\mi{FinTouch}$ of \Alg i.e. makes sure
that the third and fourth CO conditions hold for all formulas $H_k$,
$k=0,\dots,j$ built so far. However, in contrast to $\mi{FinTouch}$,
\SUb{FinTouch}{IC} does the job by inductive clauses.

We believe that \Mix is a promising algorithm for sequential
equivalence checking. One can use the relaxation described in
Section~\ref{sec:exmp} to generate an initial formula $H_j$ to be
conjoined with $P$. Constraining $P$ with $H_j$ brings one much closer
to an inductive invariant. Then some fine-tuning is done by tightening
$H_j$ with inductive clauses.




==> o3_m1ixed_alg.fig.tex <==
%
%  PC by LoR + IC
%
\setlength{\intextsep}{2pt}
%\setlength{\textfloatsep}{10pt}
%\begin{wrapfigure}{L}{2.1in}
\begin{figure}
%\begin{center}
\small
%\normalsize
%\vspace{-10pt}
\begin{tabbing}
aaa\=bb\=cc\= dd\= \kill
$\mi{PC\_LoR\_IC}(T,I,P)$ \{\\
\tb{\scriptsize{1}}\> $H_0 := I$;  \\
\tb{\scriptsize{2}}\> $j = 1$; \\
\tb{\scriptsize{3}}\>  while ($\mi{true}$) \{ \\
\tb{\scriptsize{4}}\Tt  $\trx{j-1,j} := T_{j-1,j}$; \\
\tb{\scriptsize{5*}} \Tt  $H_j := \mi{EducatGuessRlx}(\Abs{H}{j-1},\Ttrx{j})$; \\  
\tb{\scriptsize{6*}} \Tt $H_j := H_j \wedge P$; \\
\tb{\scriptsize{7*}}\Tt  $\mi{Cex} := \SUb{ThirdCOcond}{IC}(\Abs{H}{j},\ttrx{j})$; \\
\tb{\scriptsize{8}}\Tt   if ($\mi{Cex} \neq \mi{nil}$) return($\mi{No}$); \\
\tb{\scriptsize{9}}\Tt  $\mi{Inv} :=\SUb{FinTouch}{IC}(\Abs{H}{j},\ttrx{j})$ ;\\
\tb{\scriptsize{10}}\Tt  if ($\mi{Inv}$) return($\mi{Yes}$);  \\
\tb{\scriptsize{11}}\Tt  $j := j+1;$ \}\}\\
\end{tabbing} 
\vspace{-15pt}
\caption{\ti{PC\_LoR\_IC} procedure}
%\vspace{-15pt}
\label{fig:pc_lor_ic}
\end{figure}
%\end{wrapfigure}




==> p1qe.tex <==
\section{Partial Quantifier Elimination}
\label{sec:pqe}
In this section, we recall previous results on Partial Quantifier
Elimination (PQE).  Our objective here is just to help to understand a
key technique used in PC by LoR better.  In
Subsection~\ref{subsec:pqe_def}, we define the problem of partial
quantifier elimination introduced in~\cite{hvc-14}. In
Subsection~\ref{subsec:pqe_alg}, we give a high-level description of a
PQE-solver. The latter is based on the machinery of Dependency
sequents (D-sequents) that we describe in
Subsection~\ref{subsec:dep_seqs}.

%
% Subsection: QE and PQE
%
\subsection{Complete and partial quantifier elimination}
\label{subsec:pqe_def}
In this paper, by a quantified formula we mean one with
\ti{existential} quantifiers.  Given a quantified formula
\prob{W}{A(V,W)}, the problem of quantifier elimination is to find a
quantifier-free formula $A^*(V)$ such that $A^* \equiv \prob{W}{A}$.
Given a quantified formula \prob{W}{A(V,W) \wedge B(V,W)}, the problem
of \tb{Partial Quantifier Elimination} (\tb{PQE}) is to find a
quantifier-free formula $A^*(V)$ such that $A^* \wedge \prob{W}{B}
\equiv \prob{W}{A \wedge B}$.  Note that formula $B$ remains
quantified (hence the name \ti{partial} quantifier elimination). We
will say that formula $A^*$ is obtained by \tb{taking} \pnt{A} \tb{out
  of the scope of quantifiers} in \prob{W}{A \wedge B}. Importantly,
there is a strong relation between PQE and the notion of
\ti{redundancy} of a clause in a quantified formula. For instance,
solving the PQE problem above comes down to finding a set of clauses
$A^*(V)$ implied by $A \wedge B$ that makes the clauses of $A$
redundant in $A^* \wedge \prob{W}{A \wedge B}$. That is $A^* \wedge
\prob{W}{A \wedge B} \equiv A^* \wedge \prob{W}{B}$.


%
% Subsection: PQE algorithm
%
\subsection{Solving PQE by branching}
\label{subsec:pqe_alg}

In this subsection, we describe an algorithm for PQE introduced
in~\cite{hvc-14} in 2014.  We will refer to this algorithm as PQE-14.
Let $A(V,W), B(V,W)$ be Boolean formulas. Consider the problem of
finding formula $A^*(V)$ such that \pqe{W}{A}{A^*}{B}. We will refer
to a clause containing a variable of $W$ as a
\pnt{W}\tb{-clause}. PQE-14 is based on the following three
ideas. \ti{First}, finding formula $A^*$ comes down to generation of
clauses depending only on variables of $V$ that make $W$-clauses of
$A$ redundant in $A^* \wedge \prob{W}{A \wedge B}$.  \ti{Second}, the
clauses of $A^*$ can be derived by resolving clauses of $A \wedge
B$. The intermediate resolvents that are $W$-clauses need to be proved
redundant along with the original $W$-clauses of $A$.  However, since
formula $B$ remains quantified, there is no need to prove redundancy
of $W$-clauses obtained by resolving only clauses of $B$.


\ti{Third}, since proving redundancy of a clause is a hard problem,
PQE-14 uses branching. After proving redundancy of required clauses in
subspaces, the results of branches are merged. The advantage of
branching is that for every $W$-clause $C$ one can always reach a
subspace where $C$ can be trivially proved redundant. Namely, $C$ is
trivially redundant in the current subspace if a) $C$ is satisfied in
the current branch; b) $C$ is implied by some other clause; c) there
is an unassigned variable $y$ of $C$ where $y \in W$, such that $C$
cannot be resolved on $y$ with other clauses that are not satisfied or
proved redundant yet.


%
% Subsection: Dependency sequents
%
\subsection{Dependency sequents}
\label{subsec:dep_seqs}
PQE-14 branches on variables of $V \cup W$ until the $W$-clauses that
are descendants of formula $A$ are proved redundant in the current
subspace. To keep track of conditions under which a $W$-clause becomes
redundant in a subspace, PQE-14 uses the machinery of Dependency
sequents (D-sequents) developed in~\cite{fmcad12,fmcad13}. A D-sequent
is a record of the form \Dss{W}{A \wedge B}{q}{\s{C}}. It states that
clause $C$ is redundant in formula \prob{W}{A \wedge B} in subspace
\pnt{q}. Here \pnt{q} is an assignment to variables of $V \wedge
W$. If $\pnt{q}=\emptyset$, the D-sequent is called
unconditional. Derivation of such a D-sequent means that clause $C$ is
redundant in formula \prob{W}{A \wedge B} \ti{unconditionally}.  When
a $W$-clause $C$ is proved redundant in a subspace this fact is
recorded as a D-sequent. The objective of PQE-14 is to derive
unconditional D-sequents for all $W$-clauses of $A$.

A new D-sequent can be obtained from two parent D-sequents by a
resolution-like operation on a variable $y$. This operation is called
\ti{join}. When PQE-14 merges the results of branching on variable $y$
it joins D-sequents obtained in branches $y=0$ and $y=1$ at variable
$y$.  So the resulting D-sequents do not depend on $y$.  If formula $A
\wedge B$ is unsatisfiable in both branches, a new clause is generated
as a special D-sequent. This clause is obtained by resolving a clause
falsified in subspace $y=0$ with a clause falsified in subspace $y=1$
on $y$. Adding the resolvent clause makes all $W$-clauses redundant in
the current subspace.  By the time PQE-14 returns to the root of the
search tree, it has derived unconditional D-sequents for all
$W$-clauses of formula $A$.

PQE solving is work in progress and so is still lacking some important
techniques like D-sequent re-using.  In current algorithms, the parent
D-sequents are discarded as soon as they produce a new D-sequent by
the join operation. Although D-sequent re-using promises to be as
powerful as re-using learned clauses in SAT-solving, it requires more
sophisticated bookkeeping~\cite{lr_by_red} and so is not implemented
yet. In~\cite{tech_rep_ec_lor} we explained why re-using D-sequents
would bust equivalence checking by LoR. This explanation is applicable
to PC by LoR as well.



==> s0torage.tex <==
We introduce a new framework for Property Checking (PC) of sequential
circuits. It is based on a method called \tb{Lo}gic \tb{R}elaxation
(LoR). Given a safety property, PC by LoR relaxes the transition
system at hand which leads to expanding the set of reachable states.
The idea here is to compute a superset $A$ of the set of bad states
reachable \ti{only} by the relaxed system.  Set $A$ is computed for
every time frame by a technique called partial quantifier elimination.
If set $A$ of \mbox{$i$-th} time frame does not contain a bad state
and this state can be reached by \ti{the realaxed system} in $i$
transitions, this state is also reachable in $i$ transitions by the
original system. Hence the property at hand does not hold.

There are at least two reasons for developing methods for PC by
LoR. First, in PC by LoR an invariant, specifies the difference
between the behaviors of the original system and a relaxed one that
reaches all bad states.  So the complexity of PC can be drastically
reduced by finding a ``faulty'' relaxation that is a close to the
original system as possible. This is similar to equivalence checking
whose complexity strongly depends on how close the designs to be
compared are.  Second, PC by LoR can be used for proving existence of
a bug rather than finding an explicit counterexample. This feature has
the potential of improving the efficiency of bug hunting.
---------
Formula $H_j$ strongly depends on the degree of relaxation of \ksr:
the more relaxed the latter is the more states falsify $H_j$.  If
\impl{H_j}{P} does not hold, then either \Ks is buggy or \Ksr is not
sufficiently relaxed. \Alg tries to strengthen $H_j$ by adding clauses
generated to make up for relaxing even more (some) transition
relations \trx{i-1,i}, $i \leq j$ of \ksr. The process of strenthening
$H_j$ either makes the latter imply $P$ or shows that \nimpl{H_j}{P}
for any relaxation. This means that a bad state is reachable in \Ks in
$j$ transitions and $P$ does not hold.  If \impl{H_j}{P} does hold,
all bad states are reachable in $j$ transitions only by \ksr and so
$P$ is true for \Ks for $j$ transitions. Then \Alg checks if $H_j$ is
an inductive invariant.  If so, then $P$ holds for \Ks and \Alg
terminates. Otherwise, \Alg starts computing boundary formula
$H_{j+1}$.
%
----------
Our interest in PC by LoR is threefold.  First, PC by LoR can be
viewed as a version of equivalence checking of the original and
relaxed designs where one needs to compute the states reachable only
by the latter. So in a sense, the complexity of PC becomes relative
since it depends on how different the original and relaxed systems
are.  This is similar to regular equivalence checking whose complexity
strongly depends on how close the designs to be compared are. Second,
by using a particular relaxation scheme one can take into account
problem specifics. Suppose for instance, that an invariant $K$ has
been found proving that a property holds and one needs to know if the
latter still holds after a design modification. Then one can relax the
current design by adding the $K$-states to the initial states. This
way one can re-use the work done to derived invariant $K$ (assuming
that the new invariant is close to $K$). Third, PC by LoR can be used
for proving existence of a bug rather than finding it explicitly. This
feature has the potential of improving the efficiency of bug hunting.
--------
 As we show in
Section~\ref{sec:bnd_form}, a boundary formula $H_j$ satisfies the
equality \prob{\Abs{W}{j-1}}{I_0 \wedge \Abs{T}{j}} $ \equiv H_j
\wedge $ \prob{\Abs{W}{j-1}}{I_0 \wedge \ttrx{j}}.  Here 
\begin{itemize}
\item  $\Abs{W}{j-1} = W_0 \cup \dots \cup W_{j-1}$, $W_i = S_i \cup X_i \cup Y_i$, $i=0,\dots,j-1$
\item $I_0$ denotes $I(S_0)$,
\item  $\Abs{T}{j} = T_{0,1} \wedge \dots \wedge T_{j-1,j}$ 
\item  $\ttrx{j} = \Abs{T}{j-1} \wedge \trx{j-1,j}$. 
\end{itemize}
Note that formulas \prob{\Abs{S}{j-1}}{I_0 \wedge \Abs{T}{j}} and
\prob{\Abs{S}{j-1}}{I_0 \wedge \ttrx{j}} specify the sets of states
reachable in $j$ transitions in \Ks and \ksrr{j} respectively.  So
$H_j$ can be viewed as a ``boundary'' between these two sets of states
hence the name. 
--------
%
% Proposition: finding boundary formulas by induction
%
\begin{proposition}
%\label{prop:ind_bnd_form}
Let $H_j$ be a boundary formula for \ksr.  Let $H_{j+1}$ be a formula
such that $\prob{\Abs{W}{j}}{ I_0 \wedge H_j \wedge \ttrx{j} \wedge
T_{j,j+1}} \equiv H_{j+1} \wedge
\prob{\Abs{W}{j}}{I_0  \wedge \ttrx{j+1}}$.
Then $H_{j+1}$ is a boundary formula with respect to \ksr.
\end{proposition}
%
\begin{proof}[\kern-10pt Proof]
Denote formula \prob{\Abs{W}{j}}{ I_0 \wedge
H_j \wedge \ttrx{j} \wedge T_{j,j+1}} as \Fi. Let us show that
\Fii is logically equivalent to \prob{\Abs{W}{j}}{I_0 \wedge \Abs{T}{j+1}}.
Then Proposition~\ref{prop:bnd_form} entails that $H_{j+1}$ is a boundary
formula.

 Formula \Fii can be represented
as \Prob{\Abs{W}{j-1}}{W_j}{I_0 \wedge H_j \wedge \ttrx{j} \wedge
T_{j,j+1}}.  Taking into account that $T_{j,j+1}$ and $H_j$ do not
depend on variables of \Abs{W}{j-1}, one can rewrite formula \Fii as
$\exists{W_j}[T_{j,j+1} \wedge
H_j \wedge \prob{\Abs{W}{j-1}}{I_0 \wedge \ttrx{j}}]$.  Since $H_j$ is
a boundary formula, \Fii can be transformed into
$\exists{W_j}[T_{j,j+1} \wedge \prob{\Abs{W}{j-1}}{I_0 \wedge \Abs{T}{j}}]$.
After putting $T_{j,j+1}$  back under the scope of
quantifiers, \Fii becomes equal to
$\exists{W_j}[ \prob{\Abs{W}{j-1}}{I_0 \wedge \Abs{T}{j} \wedge
T_{j,j+1}}]$ and hence to
$\exists{\Abs{W}{j}}[I_0  \wedge \Abs{T}{j+1}]$.
\end{proof}
%
% Lemma: previous boundary formulas are redundant
%
\begin{lemma}
\label{lemma}
Let $H_k$ and $H_j$ be boundary formulas where $k < j$.
Then $H_j \wedge \prob{\Abs{W}{j-1}}{H_k \wedge I_0 \wedge \ttrx{j}} \equiv$
$H_j \wedge \prob{\Abs{W}{j-1}}{I_0 \wedge \ttrx{j}}$.
\end{lemma}
%
\begin{proof}[\kern-10pt Proof]
Assume the equality does not hold. Consider the two alternatives below.

\noindent $\mi{Left\_part}$ = 1, $\mi{Right\_part}$ = 0. 
This would mean that $H_k \wedge I_0 \wedge \ttrx{j}$ does not imply
$I_0 \wedge \ttrx{j}$. So we have a contradiction.

\noindent $\mi{Left\_part}$ = 0, $\mi{Right\_part}$ = 1.
 Then there is a valid trace of \Ksr reaching a state
\pnt{s_j} in $j$ transitions such that $H_j(\pnt{s_j})=1$.
 Since $H_j$ is a boundary formula this means that
\pnt{s_j} is reachable in \Ks in $j$ transitions. Then there is a 
valid trace $t = \Tr{x}{s}{0}{j}$ of \Ks reaching \pnt{s_j}.  Since
the left part evaluates to 0, then $t$ falsifies $H_k$. This is
possible only if $H_k(\pnt{s_k}) = 0$. Since $H_k$ is a boundary
formula, this means that \pnt{s_k} is not reachable in \Ks in $k$
transitions. Hence, $t$ is not a valid trace of \Ks and we have a
contradiction.
\end{proof}

%
% Proposition: Building BF by PQE
%
\begin{proposition}
%\label{prop:pqe_bnd_form}
Let $H_j$ be a boundary formula for \ksr.  Let $T_{j,j+1} =
Q_{j,j+1} \wedge \trx{j,j+1}$.  Let $H_{j+1}$ be a formula obtained by
taking $Q_{j,j+1}$ out of the scope of quantifiers $\prob{\Abs{W}{j}}{
I_0 \wedge H_j \wedge \ttrx{j} \wedge
Q_{j,j+1} \wedge \trx{j,j+1}}$. Then $H_{j+1}$ is a boundary formula
with respect to \ksr.
\end{proposition}
%
\begin{proof}[\kern-10pt Proof]
The fact that $H_{j+1}$ is taken out of the scope of quantifiers means 
that $\prob{\Abs{W}{j}}{
I_0 \wedge H_j \wedge \ttrx{j} \wedge
Q_{j,j+1} \wedge \trx{j,j+1}}$ $\equiv$ $H_{j+1} \wedge \prob{\Abs{W}{j}}{
I_0 \wedge H_j \wedge \ttrx{j}  \wedge \trx{j,j+1}}$. The right part
can be rewritten as $H_{j+1} \wedge \prob{\Abs{W}{j}}{
I_0 \wedge H_j \wedge \ttrx{j+1}}$.  Lemma~\ref{lemma} entails
that $H_j$ can be removed from the right part. So 
$\prob{\Abs{W}{j}}{
I_0 \wedge H_j \wedge \ttrx{j} \wedge
T_{j,j+1}}$ $\equiv$ $H_{j+1} \wedge \prob{\Abs{W}{j}}{
I_0  \wedge \ttrx{j+1}}$. From Proposition~\ref{prop:ind_bnd_form} it follows
that $H_{j+1}$ is a boundary formula.
\end{proof}
--------
%
% Proposition: Proving bug existence
%
\begin{proposition}
%\label{prop:bug_exst}
Let $H_j$ be a boundary formlua built for $j$-th time frame.
Let \pnt{s_j} be a bad state satisfying $H_j$, which means that $H_j$
does not imply $P$. Let trace $t=\tr{s}{0}{j}$ satisfy
$H_0 \wedge \Sub{T}{j-1}$ i.e. \pnt{s_j} is reachable in the relaxed
system in $j$ transitions.  Then \pnt{s_j} is reachable in the
original system in $j$ transitions as well and hence $P$ does not
hold.
\end{proposition}

\begin{proof}[\kern-10pt Proof]
Since $H_j$ is a boundary formula then 
$\prob{\Abs{S}{j-1}}{I_0 \wedge \Abs{T}{j-1}} \equiv H_j \wedge \prob{\Abs{S}{j-1}}{H_0 \wedge
\Abs{T}{j}}$. Since $H(\pnt{s_j})=1$, the equality above entails that 
\prob{\Abs{S}{j-1}}{I_0 \wedge \Abs{T}{j}} evaluates to 1 for assignment \pnt{s_j} to $S_j$.
That is bad state \pnt{s_j} is reachable in the original system.
\end{proof}
-------------
We will require that \Ks has the \tb{stuttering} feature i.e.  for
every state \pnt{s}, formula \Prob{X}{Y}{T(\pnt{s},X,Y,\pnt{s'})} = 1.
That is for every present state \pnt{s}, there is an input assignment
\pnt{x} such that the next state produced by circuit $N$ is also
\pnt{s}.  If \Ks does not have this feature, one can introduce
stuttering by adding to circuit $N$ one combinational input variable
$v$.  Circuit $N$ works as before if $v=1$ and copies its input
assignment to the output if $v=0$.  On the one hand, introduction of
stuttering does not affect the reachability of a bad state. One the
other hand, stuttering guarantees that \Ks has two nice properties.
First, $\prob{W}{T(S,X,Y,S')} \equiv 1$ holds where $W = S \cup X \cup
Y$.  Indeed for every next state \pnt{s'}, $T$ specifies a
``stuttering transition'' from \pnt{s} to \pnt{s'} where \pnt{s} =
\pnt{s'}.  Second, if a state is reachable in \Ks after $n$
transitions it is also reachable after any number of transitions $m$
if $m > n$.
-------
We introduce a new method for Property Checking (PC) of sequential
circuits called \Alg. Here LoR stands for \tb{Lo}gic
\tb{R}elaxation. To check that a property of a transition system holds
in \mbox{$j$-th} time frame, \Alg relaxes the transition relation.
The objective of this relaxation is to make bad states reachable by
the relaxed system in $j$-th time frame. Then \Alg computes a make-up
set specifying the states that need to be excluded to nullify the
difference between original and relaxed transition relations.  This
set is computed by a technique called partial quantifier elimination.
If a bad state is not in the make-up set, it is reachable by both
relaxed and original systems i.e. the property fails.  \Alg is
complete i.e. it either finds a bug or builds an inductive invariant.

The merit of \Alg is as follows. An inductive invariant can be viewed
as a set of constraints excluding all the bad states and some
unreachable good states. Intuitively, the ``right'' good states to be
excluded are structurally related to bad states. On the other hand,
the bad and good states made reachable by relaxing the transition
relation are structurally close. So, a make-up set contains good
states whose exclusion is structurally justified. We substantiate the
intuition above by an example with sequential equivalence checking. We
describe an algorithm based on \Alg and prove its soundness and
completeness.
-----------
An inductive invariant usually involves build a set $A_i$ (or a
sequence of such states) that overapproximates the set states
reachable in $i$ transitions.  Building $A_i$ can be viewed as finding
a set of constraints that exclude all bad states and some unreachable
good states from being in $A_i$.  Finding the right set of unreachable
good states to exclude is crucial for making a property checking
algorithm efficient. Intuitively, this set of good states should be
related to the bad states via system structure.

For instance, the outstanding performance of IC3 can be attributed to
removing bad and unreachable good states related via inductive
clauses.  PC by LoR introduces a new way to build sets $A_i$ via
transition relation relaxation and PQE. In this case, the (good and
bad) states excluded from $A_i$ are the ones that are reachable only
by a relaxed system \ksrr{i}. These states are naturally related via a
relaxation of the transition relation.  Moreover, PC by LoR allows one
to amplify structure-awareness by using relaxations that are tailored
to a transition system and property.  We substantiate these advantages
of PC by LoR in Section~\ref{sec:exmp} that describes application of
our method to sequential equivalence checking.


PC by LoR heavily relies on existence of efficient PQE solvers. So
realization of the ability of PC by LoR to take into account
formula/property structure mentioned above requires a boost in the
performance of current PQE algorithms.  We believe that such an
improvement can be achieved after implementing some crucial
techniques~\cite{tech_rep_ec_lor} and so it is just a matter of time.
-------

We will require that \Ks has the \tb{stuttering} feature i.e.  for
every state \pnt{s}, formula \Prob{X}{Y}{T(\pnt{s},X,Y,\pnt{s'})} = 1.
That is for every present state \pnt{s}, there is an input assignment
\pnt{x} such that the next state produced by circuit $N$ is also
\pnt{s}.  If \Ks does not have this feature, one can introduce
stuttering by adding to circuit $N$ an additional combinational
variable (see Section ...).
----
We also describe a version of \Alg that combines LoR with derivation
of inductive clauses~\cite{ic3}. When building formula $H_{j+1}$, \Alg
uses the LoR method to generate clauses depending on $S_{j+1}$ that
exclude every bad state \ti{unreachable} from $H_j$-states. The
machinery of inductive clauses is applied to exclude every bad state
that is \ti{reachable} from an $H_j$-state. The relation between \Alg
and IC3 is not accidental. As we show in Section~\ref{sec:tightening},
IC3 can be viewed as a special case of an algorithm that uses
transition relation tightening rather than relaxation. So a natural
extension of \Alg is an algorithm that combines relaxation and
tightenting of transition relation.
------
 A complementary approach of transition
relation tightening is discussed in Section~\ref{sec:tightening}.
--------
Besides, due to the stuttering feature, if a state
is reachable in \Ks or \Ksr in $j$ transitions, it is also reachable
there for $k$ transitions if $k > j$.
----
// $S_j$ is a set of state vars. of $j$-th time frame \\
// $I_j = I(S_j)$, $P_j = P(S_j)$, $T_{j,k} = T(S_j,S_k)$ \\
// \Abs{H}{j} = $H_0 \wedge \dots \wedge H_j$ where $H_0 \equiv 1$ \\
// ~~~~ $H_i$, $i = 1,\dots,j$ is the current boundary formula \\
// \Ttrx{j}= $\ttrx{0,1} \wedge \dots \wedge \ttrx{j-1,j}$ \\
// \Abs{S}{j} = $S_0 \cup \dots \cup S_j$ \\
-------
Let us prove this proposition by induction.

\noindent\ti{Base step}. The proposition holds if $m=0$.

\noindent\ti{Induction step}. Our induction hypothesis: if property holds
for at most $m-1$ transitions it also holds for at most $m$
transitions. Assume the contrary i.e. there is a counterexample $t
= \tr{s}{0}{k}$ of $k$ transitions where \pnt{s_k} is a bad state and
$0 < k \leq m$. By the induction hypothesis, $P$ holds for at most
$m-1$ transitions. So $k = m$.  Since \impl{H_m}{P}, then \pnt{s_m}
falsifies $H_m$ Since $H_m$ is a boundary formula, for every state
reachable by \Ks at most $m$ transitions, $H_m$ evaluates to 1. So we
have a contradiction.
-----
%
%  PC by LoR + IC
%
\setlength{\intextsep}{2pt}
%\setlength{\textfloatsep}{10pt}
%\begin{wrapfigure}{L}{2.1in}
\begin{figure}
%\begin{center}
\small
%\normalsize
%\vspace{-10pt}
\begin{tabbing}
aaa\=bb\=cc\= dd\= \kill
$\mi{PC\_LoR\_IC}(T,I,P)$ \{\\

$~~~~..... $ \\
\tb{\scriptsize{6*}}\Tt  $\mi{Cex} := \SUb{RemBdSt}{IC}(\Abs{H}{j},\Ttrx{j},P,j)$;\\
$~~~~..... $ \\
\tb{\scriptsize{9*}}\Tt  $\SUb{ThirdBFcond}{IC}(Abs{H}{j},\ttrx{j})$; \\
\tb{\scriptsize{10*}}\Tt  $\mi{Inv} :=\SUb{FinTouch}{IC}(\Abs{H}{j},\ttrx{j})$ ;\\

$~~~~..... $ \\
\end{tabbing} 
\vspace{-15pt}
\caption{\ti{PC\_LoR\_IC} procedure}
%\vspace{-15pt}
\label{fig:pc_lor}
\end{figure}
%\end{wrapfigure}
------
When building formula $H_{j+1}$, \Alg
uses the LoR method to generate clauses depending on $S_{j+1}$ that
exclude every bad state \ti{unreachable} from $H_j$-states. The
machinery of inductive clauses is applied to exclude every bad state
that is \ti{reachable} from an $H_j$-state. 
-----
 Third, we show that the machinery of inductive clauses used
by IC3 can be viewed as a special case of a PC algorithm based on
transition relation tightenting rather than relaxation.
----------
 Assume that $N$ has the stuttering
feature. As we mentioned in the introduction any sequential circuit
can be turned into a stuttering one by adding one additional
combinational input variable.
--------------
The fact that $N$ and $K$ have the
stuttering features means that $M$ has this feature as well.
----------
 Besides, the very fact that a PC method needs such
preprocessing to solve a trivial example of EC indicates of method's
deficiency (for problems of this type).
-------
\begin{definition}
\label{def:tr_relax}
Let \Ks be a system specified by transition relation $T$ and formula
$I$ specifying initial states. Let \Ksr be a relaxation of system
\ks. We will say that \Ksr is obtained by \tb{TR relaxation} if
$\Sup{I}{rlx} \equiv I$ and for every time frame $j$,
\impl{T_{j,j+1}}{\trx{j,j+1}} holds. Here TR stands for transition
relation.  We will say that a system is obtained by \pnt{j}\tb{-th}
\tb{TR relaxation} of \Ks if $T_{k,k+1} \equiv \trx{k,k+1}$, $k \neq
j$ and \impl{T_{j,j+1}}{\trx{j,j+1}}. We will denote such a system
as \ksrr{j}.
\end{definition}


==> t1ightening.tex <==
\section{Tightening Transition Relation}
\label{sec:tightening}

